Distributed Bandit Learning: Near-Optimal Regret with Efficient Communication

We study the problem of regret minimization for distributed bandits learning, in which $M$ agents work collaboratively to minimize their total regret under the coordination of a central server. Our goal is to design communication protocols with near-optimal regret and little communication cost, which is measured by the total amount of transmitted data. For distributed multi-armed bandits, we propose a protocol with near-optimal regret and only $O(M\log(MK))$ communication cost, where $K$ is the number of arms. The communication cost is independent of the time horizon $T$, has only logarithmic dependence on the number of arms, and matches the lower bound except for a logarithmic factor. For distributed $d$-dimensional linear bandits, we propose a protocol that achieves near-optimal regret and has communication cost of order $\tilde{O}(Md)$, which has only logarithmic dependence on $T$.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\subsection{Lower Bound for Multi-armed Bandits}
\label{sec:low_bound}
Intuitively, in order to avoid a $\Omega\left(M\sqrt{KT}\right)$ scaling of regret, $O(M)$ amount of communication is necessary: otherwise most of the agents can hardly do better than a single-agent algorithm. We prove this intuition in the following lower bound(which applies to the expected communication complexity of randomized protocols).
%In this subsection, we propose communication lower bound for multi-armed bandit. Our theorem shows that if we want to achieve $O(\sqrt{MKT})$ regret, communication complexity need to be at least $\Omega(M)$. This matches the communication complexity  of our elimination-based protocol except for logarithmic factors. 

\begin{theorem}
\label{thm:lowerbound}
For protocols with expected communication cost less than $M/c$, there exists multi-armed bandits instances such that total regret scales as $\Omega(M \sqrt{KT})$. Here $c=3000$. 
\end{theorem}
The proof of this lower bound is a simple reduction from single-agent bandits to multi-agent bandits, mapping protocols to single-agent algorithms (see Appendix. \ref{sec:lowerboundproof}). Since one can simulate MAB with linear bandits by setting an action set of $K$ orthogonal vectors, this directly induces a $\Omega(M\sqrt{dT})$ lower bound for linear bandits when communication cost is less than $M/c$.

We note that our results in distributed multi-armed bandits match this lower bound except for a $\log T$ factor. In this sense our protocol for multi-armed bandits is indeed communication-efficient. Moreover, since $\Omega(M\sqrt{KT})$ is achievable with no communication at all, it is essentially the worst regret for a communication protocol. Therefore, this lower bound suggests that the communication-regret trade-off for distributed MAB is a steep one: with $O\left(M\log T\right)$ communication, regret can be near-optimal; with slightly less communication ($M/c$), regret necessarily deteriorates to the worst case. %This lowerbound also implies a $\Omega(M)$ communication lower bound for linear bandits. Providing a lowerbound with dependence on $d$ would be an interesting open problem.

\subsection{Comparison of Optimism-based and Elimination-based Protocols}
In the distributed multi-armed bandit task and linear bandit task, optimism-based protocols (Protocol 1 and 2) require $O\left(MK\log M\right)$ and $O\left(M^{1.5}d^3\right)$ communication respectively. Elimination-based protocols, however, require only  $\left(M\log T\right)$ and $O\left(Md\log\log d\log T\right)$. In the regime where $T$ is not exponentially large, elimination-based protocols seem to be more communication-efficient than optimism-based protocols. In particular, the dependence on $K$ or $d$ is significantly lower; this is mostly because elimination-based protocols allocate arms to agents.

On the other hand, we also note that optimism-based protocols (Protocol 1 and 2), compared to elimination-based ones (Protocol 3 and 4), seem somewhat more natural and practical. For instance, the optimization involved in Protocol 4 is potentially much harder than the optimization used in Protocol 2. %The main idea behind elimination-based protocols is allocating arms to agents. 

%\subsection{Comparison with blah}
\subsection{Future Work}
In this work, we propose communication-efficient protocols with near-optimal worst-case regret bounds. However, this may not guarantee close-to-centralized performance for a particular instance. Adopting our results to the case where instance-dependent regret is the performance measure may be an interesting problem. Another interesting problem is providing a better communication lower bound for distributed linear bandits (in order to  achieve near-optimal worst-case regret). We conjecture that close-to-$Md$ amount of communication may be necessary, which is the case in offline distributed linear regression~\cite{zhang2013information,braverman2016communication} in the context of achieving an optimal risk rate.
%In this work, we aim to reduce communication so long as the regret bound is near-optimal. However, this may not guarantee close-to-centralized performance for a particular instance. 

It will also be great if the two design principles, namely optimism and elimination, can be combined to get the best of both worlds. Communication cost of such protocols potentially may enjoy small dependencies on timescale $T$ and size of action set ($K$ or $d$) simultaneously.

We also realize that real-world distributed systems typically suffer communication latency, and computation of the agents may be asynchronous. Therefore it would be interesting to consider protocols that tolerates latency and delays. However, we note that to some extent, the synchronous case is the hard case for regret minimization, as there are $M$ agents working in concurrent throughout the execution. If we can keep most agents and only actively run $1$ agent at a time, optimal regret can be easily achieved by simulating a single-agent algorithm, using communication less than $M$ times the space complexity of that single-agent algorithm.
